Autonomous Membership Service for Enclave Applications

Trusted Execution Environment, or enclave, promises to protect data confidentiality and execution integrity of an outsourced computation on an untrusted host. Extending the protection to distributed applications that run on physically separated hosts, however, remains non-trivial. For instance, the current enclave provisioning model hinders elasticity of cloud applications. Furthermore, it remains unclear how an enclave process could verify if there exists another concurrently running enclave process instantiated using the same codebase, or count a number of such processes. In this paper, we seek an autonomous membership service for enclave applications. The application owner only needs to partake in instantiating the very first process of the application, whereas all subsequent process commission and decommission will be administered by existing and active processes of that very application. To achieve both safety and liveness, our protocol design admits unjust excommunication of a non-faulty process from the membership group. We implement the proposed membership service in a system called AMES. Our experimental study shows that AMES incurs an overhead of 5% - 16% compared to vanilla enclave execution.

==> protocol_highlight.tex <==
\section{Protocol Highlights}
{\color{blue} \bf

%\paragraph{Communication Models.} All communications between enclaves are handled by the adversarial OS. It can re-order, delay or even drop messages at will. To account for this, we model the communication between the enclaves as follows. We assume each pair of enclaves is connected by a reliable, authenticated  point-to-point channel that does not drop any message. These channels, however, are subject to a delivery scheduler controlled by an adversary that can impose arbitrary delay (``infinity'' included) on any message of its choice. If a channel is not intervened by a malicious delivery scheduler, it delivers all message within a finite but unknown bounded delay (i.e., partially synchronous). The adversary can intervene any channel and make it asynchronous.

%
%\paragraph{Faulty vs. Live and Active Enclaves.} We call an enclave ``faulty'' if it has crashed. We call an enclave ``live'' if it is not faulty. A live enclave whose existence is questioned by other enclave, potentially because its communications channels are blocked by the adversarial delivery scheduler, are ``inactive''. Otherwise, the enclave is ``active''. A inactive enclave may become active again if it can fetch all necessary information from other active and correct enclaves, and update its internal state accordingly.  Let $n$ be a total number of enclaves registered in the system, and $f$ be the number of faulty and inactive enclaves. In order for the system to remains operational, it must be the case that $f \leq \frac{n-1}{2}$. If $f$ exceed $\frac{n}{2}$, the system should halt (i.e., the remaining $n-f$ correct enclaves commit suicide).

%
%\paragraph{Consensus protocol}. A consensus protocol run among a set of $n$ nodes, and tolerate $f \leq \frac{n-1}{2}$ faulty nodes. It has two main property:
%
%\begin{itemize}
%\item Safety: Let $act$ be the value to be agreed upon. When the protocol completes, if a correct node accepts $act$, all other correct nodes accept $act$~\footnote{Based on the ``commit'' messages a node receives during the consensus protocol, it knows who would agree with it. Nonetheless, it does not know if the same $act$ are carried out at those nodes, for the other node can crash immediately after sending that ``commit'' message.}.
%
%\item Liveness: We call the protocol ``live'' if it can make progress (i.e., correct nodes are not stuck at processing a certain $act$ value forever).
%
%\end{itemize}

%\paragraph{Enclave's internal state.} 
%Each enclave $[i]$ maintain two lists: $M_i$ comprises identity of all enclaves that $i$ believes to be ``registered'', and $A_i$ comprises identity of enclaves $[i]$ believes to be ``alive''. Let us assume the limit on the number of concurrently running enclave is $L$, it must always be the case that $|M_i| < L$. $[i]$ will remove an enclave $[j]$ from its $A_i$ list if it does not listen from $[j]$ before its (countdown) timer against $[j]$, denoted by $D_{i \cdot j}$, elapses.
%Each enclave progresses in ``epochs'' with duration $D$ according to its own clock. \\

\paragraph{Membership Services}.
We follow Raft's strategy in maintaining the membership information among the enclave instances. Let $n$ denotes the current number of registered enclaves in the system. One enclave is designated as the ``Leader'', and the remaining [n-1] are ``Follower''. The Leader needs to exchange heartbeats with the Followers, to maintain its leadership and to detect if a Follower has crashed. In normal case (i.e., when the Leader is active and operates correctly), Followers need not exchange heartbeats with one another. 

%\noindent [Follower crashes]. If the Leader detects a Follower $j$ has crashed, it drives all other followers to remove $j$ from their peer-list. 
%\begin{itemize}
%\item Leader puts an entry $\langle down, j \rangle$ to its log. 
%\item Leader broadcast $\langle down, j \rangle$ to all Followers. Upon receiving $\langle down, j \rangle$, a Follower $i$ acknowledges the receipt by sending $\langle ack_i, down, j \rangle$ to the Leader, and puts $\langle down, j \rangle$ to its log.
%\item Once Leader has collected a majority of $\langle ack_i, down, j \rangle$, its removes $j$ from its peer-list.
%It announces this removal (a.k.a ``commit'') in the next message it exchanges with the Followers. Once the Follower sees the ``commit'', they remove $j$ from their peer-list. 
%\end{itemize}


%\noindent [New Follower]. Once the new enclave has been instantiated, the OS routes a new-enclave-joining request to the Leader. The Leader attests the new enclave, and checks if it can be added (i.e., if quota has not been consumed), and informs all Followers on the new member.
%
%\begin{itemize}
%\item Leader puts an entry $\langle add, [newID] \rangle$ to its log. 
%\item Leader broadcast $\langle add, [newID] \rangle$ to all Followers. Upon receiving $\langle add, [newID] \rangle$, a Follower $i$ acknowledges the receipt by sending $\langle ack_i, add, [newID] \rangle$ to the Leader, and puts $\langle add, [newID] \rangle$ to its log.
%\item Once Leader has collected a majority of $\langle ack_i, add, [newID] \rangle$, its adds $[newID]$ to its peer-list, and transfers to $[newID]$ all necessary information to start operating. The Leader announces this ``commit'' in the next message it exchanges with the Followers. Once the Follower sees the ``commit'', they adds $[newID]$ to their peer-list. 
%\end{itemize}


%\noindent [Suspected Leader Crash]. If a Follower does not receive any message from the Leader within a pre-determined time-out, its broadcast RequestVote message to all Followers. Upon receiving RequestVote from $i$, a Follower $j$ responds as follows:
%
%\begin{itemize}
%\item If $j$ has recently receives a message from the Leader (i.e., its timeout has not expired), it will informs $i$ that the Leader is still active. 
%
%\item Else if $j$ has voted for another ``candidate'' (potentially itself), and $i$ does not ``outweigh'' the ``candidate'' $j$  has voted for, $j$ does not switch its votes, but rather informs $i$ on the ``candidate''.
%The notion of ``outweigh'' here follows from the election criteria defined in Raft. 
%
%\item Else if $j$ has not voted for any one, or if  $i$ ``outweighs'' the ``candidate'' $j$  has voted for, $j$ grants its vote for $i$. 
%
%\end{itemize}
%Once $i$ has collected a quorum of votes (i.e., $\frac{n+1}{2}$), it assumes the role of the Leader. If $i$ cannot gather a quorum of votes within a certain time-out, it commits suicide.
%
%\noindent\textit{Remark.} If the Leader indeed crashes, no new instances can be added, and no Follower crashes can be detected during the period when the system is in the leader election state. 

%
%\noindent [Shutdown] The client can shut all instances down by sending a request to the Leader. The Leader follows Raft to informs all followers on the shutdown. 
%
%\begin{itemize}
%\item Leader puts an entry $\langle RequestShutdown \rangle$ to its log. 
%\item Leader broadcast $\langle RequestShutdown \rangle$ to all Followers. Upon receiving $\langle RequestShutdown \rangle$, a Follower $i$ acknowledges the receipt by sending $\langle ack_i, RequestShutdown \rangle$ to the Leader, and puts $\langle RequestShutdown \rangle$ to its log.
%\item Once Leader has collected a majority of $\langle ack_i, RequestShutdown \rangle$, it broadcasts a $\langle CommitShutdown \rangle$ to all Followers. Upon receiving $\langle CommitShutdown \rangle$, a Follower $i$ acknowledges the receipt by sending $\langle ack_i, CommitShutdown \rangle$ to the Leader, and then commits suicide. 
%\item Once Leader has collected a majority of $\langle ack_i, CommitShutdown \rangle$, it informs the client, and then commits suicide.
%\end{itemize}
%}

%
%
%\noindent [ONLINE-CHECK]
%\begin{itemize}
%\item At the beginning of each epoch, $A_i = M_i$, and an enclave $[i]$ broadcasts to all enclaves in its $M_i$ list a message $\langle ping, H(M_i) \rangle$. 
%\item Upon receiving the ping message from $[i]$, enclave $[j]$ resets its timer of $[i]$ (i.e., $D_{j \cdot i}$), and responds with $\langle ack, H(M_j) \rangle$. If $[j]$ has not seen $H(M_i)$ before,  $[j]$ knows that its $M_j$ is not up-to-date. In that case, it fetches the latest member list from $[i]$. 
%
%\item Likewise, upon receiving the ack message $\langle ack, H(M_j) \rangle$, $[i]$ resets its timer of $[j]$ (i.e., $D_{i \cdot j}$), and also checks if it has seen $H(M_j)$ before. It requests for the latest member list from $[j]$ if it has not. 
%\item At the end of the epoch, if $[i]$ did not hear from a majority of its $A_i$, it commits suicide. Else $[i]$ initiates a REMOVE-MEMBER protocol for enclave $[j] \in (M_i - A_i)$. 
%Let us denote the initiation message by $\langle dead, [j] \rangle$ \footnote{If we are to treat this message as pre-prepare message in PBFT, we run into a problem of ``many primary proposing the same pre-prepare message'', as various enclaves can detect the death of $[j]$ and attempts to initiate REMOVE-MEMBER protocol independently and simultaneously. Instead, an enclave would treat the first $\langle dead, [j] \rangle$ message it receives as pre-prepare if it has not by itself suspected that $[j]$ is faulty. Otherwise, it treat $\langle dead, [j] \rangle$ as a prepare message. This does not compromise safety of the protocol, because the primary in PBFT does not send prepare, and the $2f+1$ quorum needed to move to commit phase counts both prepare and pre-prepare message.}.
%\end{itemize} 
%
%\noindent [REMOVE-MEMBER] is based on a consensus protocol. 
%\begin{itemize}
%\item Upon receiving $\langle dead, [j] \rangle$, an enclave $[i]$ checks if $[j] \in A_i$. If so, it queues the message for a maximum duration of $2D$. Otherwise, it participates in the REMOVE-MEMBER protocol against $[j]$.
%
%\item If the REMOVE-MEMBER protocol against $[j]$ succeeds, $[i]$ removes $[j]$ from $M_i$.
%
%\item While $[i]$ is queuing $\langle dead, [j] \rangle$, if it receives any message from $[j]$, $[i]$ discards the $\langle dead, [j] \rangle$ message from its queue. 
%
%\end{itemize}
%After all, [REMOVE-MEMBER] depends on partial synchrony assumption to make progress (i.e., all correct enclaves agree to remove a faulty enclave from their $M_i$. This dependence does not weaken the security of the system, for we enforce enclave suicide if in case of complete asynchrony.
%
%\noindent [ADD-MEMBER] is based on a consensus protocol. The OS routes a new-enclave-joining request to an ``authority'' enclave, who serves as a ``primary'' that initiates the ADD-MEMBER protocol among all other enclaves. The authority enclave is determined based on the hash of its ID (e.g., the enclave that has smallest $H(ID)$ is the authority enclave). Since all correct enclaves should have the same view of $M_i$, their perception of authority enclave should be consistent. Besides, we do not need view-change protocol to deal with faulty primary as in conventional PBFT, for a faulty primary will be removed via the [REMOVE-MEMBER], and the next enclave that has smallest $H(ID)$ would take over the primary role.
%
%\begin{itemize}
%\item The authority enclave $[i]$ checks if $|M_i| < L$. If so, it initiates the ADD-MEMBER protocol by broadcasting $\langle add, [newID] \rangle$. Otherwise, it ignores the request.
%
%\item Upon receiving, $\langle add, [newID] \rangle$, an enclave $[j]$ checks if $|M_j| < L$. If so, it participates in the ADD-MEMBER protocol. Otherwise, it queues the message for duration of $c \dot D$, for some constant $c$. If there is a REMOVE-MEMBER protocol succeeds before $\langle add, [newID] \rangle$ is discarded, $[j]$ participates in the ADD-MEMBER protocol for $[newID]$.
%
%\item If the ADD-MEMBER protocol for $[newID]$ succeeds, $[j]$ adds $[newID]$ to its $M_j$.
%
%\end{itemize}


%\noindent [SHUTDOWN-NOTICE] is based on a consensus protocol. When the client wants to shutdown all enclaves, he sends a request to the cloud, which then routes the request to an ``authority'' enclave determined following the same way as in ADD-MEMBER protocol.
%
%\begin{itemize}
%\item The authority enclave $[i]$ first responds the client which $|M_i|$. It then initiates the SHUTDOWN-NOTICE protocol among all other enclaves.
%
%\item All enclaves participate in the SHUTDOWN-NOTICE protocol. An enclave $[j]$ sends a shutdown-confirmation to the client, and then commit suicide.
%
%\item When the client receives $\frac{M_i + 1}{2}$ shutdown-confirmations, she is certain that her application has been shutdown.
%
%\end{itemize}
%
%\noindent [BOOTSTRAP]
%
%
%The bootstrap happens as follows:
%\begin{itemize}
%\item First enclave E1: attested by the client. After attestation, client provisions secret to the enclave.
%
%\item Second enclave E2: After instantiated, the second enclave contacts the first enclave for attestation. The attestation serves as the 1st phase in the 2PC protocol, letting E1 know that E2 is ready. Next, E1 sends the secret to E2, and E2 confirms receipt of the secret. 
%
%
%
%\item Third enclave E3: E1 performs attestation of E3, and at the same time query E2 if it is okay to add E3. This serves as the 1st phase in 2PC protocol, allowing E1 to check if both E2 and E3 are ready. Next, E1 sends secret to E3, waiting for the acknowledgement. Once receiving the acknowledgement from E3, E1 informs E2 on E3's joining. 
%
%
%\end{itemize}
%
%
%\noindent\textit{Remark.} 3PC is not necessary here. If both leader E1 and follower E2 crashes, the system stop operating anyway. Thus, there is no need to avoid ``blocking'' case of 2PC.
%
%}
